Particle Mesh Ewald for Molecular Dynamics in OpenCL on an FPGA Cluster

Molecular Dynamics (MD) simulations play a central role in physics-driven drug discovery. MD applications often use the Particle Mesh Ewald (PME) algorithm to accelerate electrostatic force computations, but efficient parallelization has proven difficult due to the high communication requirements of distributed 3D FFTs. In this paper, we present the design and implementation of a scalable PME algorithm that runs on a cluster of Intel Stratix 10 FPGAs and can handle FFT sizes appropriate to address real-world drug discovery projects (grids up to $128^3$). To our knowledge, this is the first work to fully integrate all aspects of the PME algorithm (charge spreading, 3D FFT/IFFT, and force interpolation) within a distributed FPGA framework. The design is fully implemented with OpenCL for flexibility and ease of development and uses 100 Gbps links for direct FPGA-to-FPGA communications without the need for host interaction. We present experimental data up to 4 FPGAs (e.g., 206 microseconds per timestep for a 65536 atom simulation and $64^3$ 3D FFT), outperforming GPUs. Additionally, we discuss design scalability on clusters with differing topologies up to 64 FPGAs (with expected performance greater than all known GPU implementations) and integration with other hardware components to form a complete molecular dynamics application. We predict best-case performance of 6.6 microseconds per timestep on 64 FPGAs.

==> acknowledgements.tex <==
\section{Acknowledgments}
We would like to thank several individuals at Intel, especially Nick Finamore Jr. and Nadav Zinger for their support of this project, including providing loaner hardware as well as discussions and debugging support that was provided. We would also like to thank Molex (Kenneth Robertson and Gildas Genest) for providing hardware, instructions and debugging support of 520N-MX boards.  






==> artifactdescription.tex <==
Are there computational artifacts such as datasets, software, or hardware associated with this paper?
====================================
YES

AD/AE Details
==============
Hardware Environment

We use a single dual-processor server with two 8-core Intel Xeon Silver 4110 CPUs at 2.10 GHz and 768 GB RAM,  The system is equipped with four BittWare 520N-MX FPGA modules, each with four 100 Gbps communications links.  The modules are interconnected with QSFP28 optical cables using point to point wiring.

Software Environment

The server runs CentOS 7.7, with a Linux 3.10.0-957 kernel.  Software development uses GCC 6.3.0.  FPGA development uses Intel Quartus Pro 19.3.  The FPGA boards are running the BittWare p520\_max\_m210h board support package. Python 2.7.15 is used for some preprocessing and OpenCL code generation, and PyOpenCL for interactive experimentation.  FFTW3 used for comparison.  OpenCL FFT core from https://www.intel.com/content/www/us/en/programmable/support/support-resources/design-examples/design-software/opencl/fft-2d.html


Methodology

Timings reported in the paper are obtained by measuring elapsed wall clock time in the host program from just before the invoking call to clEngueueTask to just after the completion of the call to clFinish.  Timing runs are modified to loop 1000 times inside the OpenCL code to create manageable measurement intervals.  Testing is done with C++ host programs.

GPU FFT timings were obtained using nVidia cuFFT 9.1

FFT performance is not data-dependent.  Data sets used are IID complex values with real and complex parts in the range [-1..1].  Correctness evaluated with FFTW3.



Artifacts Available (AA)
==========================

Software Artifact Availability. SOME

Hardware Artifact Availability: THERE ARE NONE

Data Artifact Availability: THERE ARE NONE

Proprietary Artifacts: THERE ARE SOME


Experimental setup 
G==================

Hardware Details: dual  8-core Intel Xeon Silver 4110 CPUs at 2.10 GHz and 768 GB RAM, four BittWare 520N-MX FGPA accelerators

OS Versions:  CentOS 7.7, with a Linux 3.10.0-957 kernel

Compilers and versions: GCC 6.3.0, Intel FPGA SDK 19.3, Bittware p520_max_m210h

Key Algorithms: 3D FFT, Ewald Summation

Input Datasets: Random single precision complex data

Artifact Evaluation
====================

Are you completing an Artifact Evaluation (AE) Appendix?  NO


==> bibliography.tex <==

\section{Things to cite somewhere}

Martin's FFT paper
Anton FFT paper
FFTW
Parallel pipelined FFT paper
Bit reversal paper?
Vector radix paper
OpenCL info?


@article{key ,
author = {Mario Garrido and J. Grajal and M.A. Sanchez and and Oscar Gustafsson}, title = {Pipelined Radix-$2^k$ Feedforward FFT Architectures},
journal = {IEEE Transactions on Very Large Scale Integration Systems}, volume = {21},
year = {2013},
number = {1},
pages = {23--32},
doi = {10.1109/TVLSI.2011.2178275}
}



@ARTICLE{6118316, author={M. {Garrido} and J. {Grajal} and M. A. {Sanchez} and O. {Gustafsson}}, journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems}, title={Pipelined Radix-$2^{k}$ Feedforward FFT Architectures}, year={2013}, volume={21}, number={1}, pages={23-32},}

@article{garrido2011pipelined,
  title={Pipelined radix-$2\^{}$\{$k$\}$ $ feedforward FFT architectures},
  author={Garrido, Mario and Grajal, Jes{\'u}s and Sanchez, MA and Gustafsson, Oscar},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={21},
  number={1},
  pages={23--32},
  year={2011},
  publisher={IEEE}
}

@ARTICLE{8589011, author={M. {Garrido} and K. {Möller} and M. {Kumm}}, journal={IEEE Transactions on Circuits and Systems I: Regular Papers}, title={World’s Fastest FFT Architectures: Breaking the Barrier of 100 GS/s}, year={2019}, volume={66}, number={4}, pages={1507-1516},}

@article{garrido2018world,
  title={World’s Fastest FFT Architectures: Breaking the Barrier of 100 GS/s},
  author={Garrido, Mario and M{\"o}ller, Konrad and Kumm, Martin},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers},
  volume={66},
  number={4},
  pages={1507--1516},
  year={2018},
  publisher={IEEE}
}

@ARTICLE{8633387, author={M. {Garrido} and J. {Grajal} and O. {Gustafsson}}, journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems}, title={Optimum Circuits for Bit-Dimension Permutations}, year={2019}, volume={27}, number={5}, pages={1148-1160},}

@article{garrido2019optimum,
  title={Optimum circuits for bit-dimension permutations},
  author={Garrido, Mario and Grajal, Jes{\'u}s and Gustafsson, Oscar},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={27},
  number={5},
  pages={1148--1160},
  year={2019},
  publisher={IEEE}
}

@inproceedings{10.1145/3295500.3356179, author = {Yang, Chen and Geng, Tong and Wang, Tianqi and Patel, Rushi and Xiong, Qingqing and Sanaullah, Ahmed and Wu, Chunshu and Sheng, Jiayi and Lin, Charles and Sachdeva, Vipin and Sherman, Woody and Herbordt, Martin}, title = {Fully Integrated FPGA Molecular Dynamics Simulations}, year = {2019}, isbn = {9781450362290}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/3295500.3356179}, doi = {10.1145/3295500.3356179}, booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis}, articleno = {Article 67}, numpages = {31}, keywords = {molecular dynamics, high-performance computing, FPGA}, location = {Denver, Colorado}, series = {SC ’19} }

@article{eastman2010openmm,
  title={OpenMM: A hardware-independent framework for molecular simulations},
  author={Eastman, Peter and Pande, Vijay},
  journal={Computing in science \& engineering},
  volume={12},
  number={4},
  pages={34--39},
  year={2010},
  publisher={IEEE}
}
article{eastman2017openmm,
  title={OpenMM 7: Rapid development of high performance algorithms for molecular dynamics},
%  author={Eastman, Peter and Swails, Jason and Chodera, John D and McGibbon, Robert T and Zhao, Yutong and Beauchamp, Kyle A and Wang, Lee-Ping and Simmonett, Andrew C and Harrigan, Matthew P and Stern, Chaya D and others},
  author={Eastman, Peter and others},
  journal={PLoS computational biology},
  volume={13},
  number={7},
  pages={e1005659},
  year={2017},
  publisher={Public Library of Science}
}



@article{key ,
author = {Mario Garrido and J. Grajal and M.A. Sanchez and and Oscar Gustafsson}, title = {Pipelined Radix-$2^k$ Feedforward FFT Architectures},
journal = {IEEE Transactions on Very Large Scale Integration Systems}, volume = {21},
year = {2013},
number = {1},
pages = {23--32},
doi = {10.1109/TVLSI.2011.2178275}
}



@ARTICLE{6118316, author={M. {Garrido} and J. {Grajal} and M. A. {Sanchez} and O. {Gustafsson}}, journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems}, title={Pipelined Radix-$2^{k}$ Feedforward FFT Architectures}, year={2013}, volume={21}, number={1}, pages={23-32},}

@article{garrido2011pipelined,
  title={Pipelined radix-$2\^{}$\{$k$\}$ $ feedforward FFT architectures},
  author={Garrido, Mario and Grajal, Jes{\'u}s and Sanchez, MA and Gustafsson, Oscar},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={21},
  number={1},
  pages={23--32},
  year={2011},
  publisher={IEEE}
}

@article{garrido2018world,
  title={World’s Fastest FFT Architectures: Breaking the Barrier of 100 GS/s},
  author={Garrido, Mario and M{\"o}ller, Konrad and Kumm, Martin},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers},
  volume={66},
  number={4},
  pages={1507--1516},
  year={2018},
  publisher={IEEE}
}

@article{garrido2019optimum,
  title={Optimum circuits for bit-dimension permutations},
  author={Garrido, Mario and Grajal, Jes{\'u}s and Gustafsson, Oscar},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={27},
  number={5},
  pages={1148--1160},
  year={2019},
  publisher={IEEE}
}

@inproceedings{10.1145/3295500.3356179, author = {Yang, Chen and Geng, Tong and Wang, Tianqi and Patel, Rushi and Xiong, Qingqing and Sanaullah, Ahmed and Wu, Chunshu and Sheng, Jiayi and Lin, Charles and Sachdeva, Vipin and Sherman, Woody and Herbordt, Martin}, title = {Fully Integrated FPGA Molecular Dynamics Simulations}, year = {2019}, isbn = {9781450362290}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/3295500.3356179}, doi = {10.1145/3295500.3356179}, booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis}, articleno = {Article 67}, numpages = {31}, keywords = {molecular dynamics, high-performance computing, FPGA}, location = {Denver, Colorado}, series = {SC ’19} }

@article{eastman2010openmm,
  title={OpenMM: A hardware-independent framework for molecular simulations},
  author={Eastman, Peter and Pande, Vijay},
  journal={Computing in science \& engineering},
  volume={12},
  number={4},
  pages={34--39},
  year={2010},
  publisher={IEEE}
}
article{eastman2017openmm,
  title={OpenMM 7: Rapid development of high performance algorithms for molecular dynamics},
  author={Eastman, Peter and Swails, Jason and Chodera, John D and McGibbon, Robert T and Zhao, Yutong and Beauchamp, Kyle A and Wang, Lee-Ping and Simmonett, Andrew C and Harrigan, Matthew P and Stern, Chaya D and others},
  journal={PLoS computational biology},
  volume={13},
  number={7},
  pages={e1005659},
  year={2017},
  publisher={Public Library of Science}
}

@BOOK{Tolimieri:fft,
  AUTHOR = "R. Tolimieriand M. An and C. Lu",
  TITLE = "Algorithms for Discrete Fourier Transform and Convolution",
  PUBLISHER = "Springer-Verlag",
  ADDRESS = "New York",
  YEAR = "1989"
}

@MANUAL{IntelSDK,
  title =        {{Intel\textregistered FPGA SDK for OpenCL\textsuperscript{TM} Pro Edition}},
  author =       {{Intel Corporation}},
  month =        {April},
  year =         {2020},
  note =         {\url{https://www.intel.com/content/dam/www/programmable/us/en/pdfs/literature/hb/opencl-sdk/aocl_programming_guide.pdf}}
}

@MANUAL{nvidia:cufft,
  title =        {{nVidia\textregistered cuFFT}},
  author =       {{nVidia Corporation}},
  month =        {January},
  year =         {2021},
  note =         {\url{https://developer.nvidia.com/cufft}}
}


@MANUAL{nvidia:v100,
  title =        {{nVidia\textregistered V100}},
  author =       {{nVidia Corporation}},
  month =        {January},
  year =         {2021},
  note =         {\url{https://www.nvidia.com/en-us/data-center/v100/}}
}


==> changes.tex <==
Statement of changes

Major issues: 
1) Lack of MD results - The purpose of the paper is demonstration of scalable 3D FFT.  The motivation for that work is a full FPGA-based production MD code, but we're not yet ready to report on it. We've reworked the Introduction and background in an attempt to avoid overpromising.  We also added a new section about how the FFT fits into the overall MD problem. As reviewer 1 points out, merely remoting the FFT would cause excessive host-fpga traffic and could not perform well  The problem is not so much serialization from Amdahl's law as a sheer lack of host bandwidth compared to the 300 GB/s or so we are able to achieve on each FPGAs.  The changes (we hope) make clear that we plan to run entire sequences of timesteps without host interaction.

We've tried to clean up the explanation of the Fourier methods for Ewald summation.  In short we're using SPME, with one forward and one inverse FFT per timestep, with the FT of the Greens function computed ahead of time on the host and stored in RAM on the FPGAs for use over multiple time steps. "tabulated" in the language of "How to Convert SPME to P3M"

2) Comparison to Anton:
Anton 1's 3D FFT performance, after over 10 years, remains unparalleled. As such it remains one of the very few published 3D FFT results with which we can compare. Mostly due to advances in circuits, and partly due to our efforts, we can now approach Anton 1's FFT performance on a single FPGA and at least on paper, should do better with 8 FPGAs or up.  Anton 2 changed focus to mu-series real-space convolutions, citing a 15 percent performance improvement in trade for additional communications.  We <think> we know how to scale FFT further and can leverage the availability of OpenMM's PME (really SPME) code. With the publication of the mu-series paper in J Chem Phys in February 2020 it may become more widely used and we'll continue to track it.

3) Use of OpenCL

We added a section on the selection of OpenCL and some of our experience.  It's good for reasonably fast development but offers abstractions that tend to hide the power of the hardware. We're actually not targetting performance portability, but rather trying to use OpenCL to create a specific thing: a fast scalable 3D FFT on FPGA that can be integrated easily with a full MD application.

4) Where the FFT work fits in the context of MD

We added a section Molecular Dynamics on Multiple FPGAs. The overall setup is shown in Figure 1, with the 3D FFT as parts of the Long Range force Pipeline, interacting with short range and bonded force pipelines that use spatial decomposition for scaling.  Pipeline coordination and particle migration are handled by Motion Update and Force Accumulator modules which we do not describe in this paper.  We added a figure showing the planned 4-fpga layout of the full application.

5) Energy consumption.
We're unable to provide energy data yet, because we're running early versions of the board support packages and energy reporting is not available.

Other changes

a) Added a section on planned complete molecular dynamics on FPGAs along with some details on our hort range and non-bonded work as well (which we have not covered in this paper) on page 9. This section summarizes our design of heterogeneous execution on multiple FPGAs. Our planned design does not include any communication between the CPU and the FPGA. 
b) Added section on "FPGA Programming using OpenCL" which details our experience using OpenCL for programming FPGAs on page 9. This section talks about our reason of using OpenCL, issues facing OpenCL and features that are lacking in OpenCL as well. 
c) Added text on pages 2 and 9 to summarize the mu-series implementation and why it might not be a good match for the FPGA architecture. 
d) Reworded introduction to reduce the stress on MD; our connection to MD is that the sizes here are applicable to molecular dynamics for small molecule drug discovery, and that the FFT is included in the long range pipeline for molecular dynamics. 
e) Eliminated Section on 3D FFT Schedules as uninformative to readers.
f) Added citations suggested by reviewers and some others
g) Verify that bram fft is in correct section, and that the HBM pipe is shown. Minor edits, like fixing double quotes.
h) Gave a reason for not including energy usage as well as issues running long-range pipeline due to COVID19 disruptions. 
i) Rework layout of Table III, IV for readability
j) Increase font size in graphics for readability
k) Made Table I and Table II span two columns for readability
l) Made substantial improvements to the Artifact Description, per reviews

Additions are marked in blue text.  Deletions are mentioned here. 



==> combinedmd.tex <==

\section{Molecular Dynamics on Multiple FPGAs}\label{sec:multi_fpga_md}
%At the time of writing this paper, we have been unable to execute long-range pipelines on actual hardware. This currently requires hardware and FPGA connection debugging, which currently can only be performed in person. This has been a bottleneck due to COVID-19 related restrictions on movement. 

Our ultimate goal is to perform multiple timesteps of the full MD application on a network of FPGAs without any additional host communication beyond initialization and result collection. This architecture is shown in Figure~\ref{fig:MDOverview}. Required MD functionality must include: short-range, long-range and bonded force calculations, motion integration, on-chip particle data storage and management, etc.~\cite{yang2019fully}. %In this paper, we focus on 3DFFT and its use in long-range force calculation while other aspects are the focus of current and future work. We chose FFT instead of the $\mu$-series that Anton 2 implemented \cite{shaw2014anton}. At the time of implementation, it was not clear to us if $\mu$-series will give us benefits on the FPGA. The $\mu$-series seems to increase communication requirements, and therefore this algorithm might be better suited for the Anton-2 architecture and in any case a fast FFT is useful for a variety of problems in addition to MD. 

As the required on-chip resources for problem sizes of interest (e.g., 64k-128k atom simulations) exceed that which is available for a single target FPGA, we must employ some degree of resource sharing and/or circuit partitioning across multiple FPGAs to achieve the required performance. We use a straight-forward spatial decomposition scheme to partition work across multiple FPGAs. The short-range and bonded force pipelines operate on nearby particles, with particle migration handled by a motion update module (see Figure~\ref{fig:MDOverview}). Given a fixed problem size, as we increase the number of FPGAs, the required resources per FPGA will decrease. For a high number of FPGAs, there are sufficient resources per FPGA to employ a homogeneous design (i.e., all MD functionality for a given sub-region of simulated space is performed on the same FPGA). For a low number of FPGAs (e.g., 4-8), this is not the case and we must employ a heterogeneous design. This design will assign long-range pipelines to a subset of FPGAs, with all other functionality assigned to the remaining FPGAs. This approach is similar to, and inspired by, the parallelization strategy used in GROMACS~\cite{Gromacs2020}. A diagram is shown in Figure~\ref{fig:multifpga}.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{SC_2020/diagrams/multifpga.pdf}
  \caption{Full MD algorithm on 4 FPGAs.}
  \label{fig:multifpga}
  \vspace{-10pt}
\end{figure}


Data communication between long-range and other pipelines is performed through QSFP channels, which directly communicate between FPGAs without coordinating with the host. The communication interface to/from the LR pipeline is a stream of atom positions and charges to and a stream of atom force updates from the pipelines. Although, we ultimately plan to construct a 64-FPGA cluster configured as a $4^3$ 3D-torus, our initial target of a 4-FGPA prototype is configured as 2 FPGAs with 2 LR pipelines each and the other 2 FPGAs are reserved for the rest of the application. With this configuration, we can support four atoms per cycle and four force updates per cycle, which matches the capability of the LR pipeline design to accept data and deliver results without processing delays. We balance the performance of the various pipelines to minimize the maximum runtime and thus minimize the timestep execution time.

%These 


%Any fine-grained communication running on the FPGA functions running on the host will severely curtail performance of the FPGA implementation, and therefore, it is essential that all molecular dynamics functions be moved to the FPGA. 
%we need multiple pipelines to get speedup compared to other architectures, which in turn leads to more resource utilization.


==> extra.tex <==

LCS Move the following paragraph later

A convenient way to express the data ordering is by a data address permutation that addresses the data first by parallel lane and then by clock cycle.  In this notation, the FFT input is in the order X4 X3 X2 X0 X1 and the output is in order X4 X3 X2 X1 X0. These string descriptions are given lowest order bit first.  The first three bits describe 8 parallel lanes and later bits show the time sequencing of words.

LCS move next two PP later

Implementation of a distributed FFT is a complex tradeoff among compute resources on each platform, the data layout across devices, and the communications resources available.

In the case of molecular dynamics, it is desirable to minimize compute resources in order to leave the most device area for the rest of the problem.


\section{FFT}

One D FFT
3D FFT
Vector-radix FFT

FFT generator IP for FPGAs
OpenCL FFT modules

Chart of size v datatype vs bandwidth v networking

Transpose problem
Memory bandwidth



\subsection{A single pipeline

\subsection{History}

When we began the FPGA project in the spring of 2019, we had a single Bittware 520N board available, containing Intel Stratix 10 28xxG parts with two banks of DDR memory and 4 40 Gbps QSFP communications links.  Since then, we have moved to four Molex p520\_MAX\_m210h boards with Intel Stratix 10 28xxxH parts, 32 banks of High Bandwidth Memory, and 4 100 Gbps links.  Our testbed currently consists of four FPGA boards. Two QSFP ports are used to configure a 1D ring network, and the other two QSFPs connect to boards which are two hops away. This arrangement permits both four board fully connected configurations and two board configurations with two direct links.


The DDR based Stratix 10 board has available about 80 GB/second of memory bandwidth.  We tested some fairly simple computational kernels and were able to run one load-store pipeline at 16 GB/sec (32 GB/s total).  Two simultaneous pipelines were able to achieve about 50 GB/s total). This limited our ability to test large numbers of pipelines until the HBM modules became available

Each HBM module has 32 independent banks of HBM memory, each with a 256 bit wide interface.  We use these as striped pairs to obtain 512 bit interfaces for 8-way parallel single precision floating point.  Each memory to memory FFT pipeline requires four banks, with an optional fifth bank for the full long range pipeline to read Green's function data.

Due to the technology of dynamic memory, there is a natural advantage to accessing memory in order.  According to the Intel guidance, one should be able to achieve full bandwidth with 64 byte-wide references provided that 16 accesses are made in order, for a total of 1024 bytes.


\subsection{Networking}

The 520N modules support 4 QSFP28 serial ports, each running at 100 Gbps.  The next generation is expected to support 400 Gbps ports. With four ports per FPGA, one is naturally inclined to implement a 2D torus network.  With six ports per FPGA, a 3D torus network becomes possible.  We plan to investigate use of Oculink connectors present on the boards to implement two additional copper links for a third dimension.

Parallelizing 3D FFT is challenging because while one can compute many of the X and Y dimension transposes in parallel, they must exchange data in an All to All pattern with every other instance.  As an example, if one divides the 3D volume along the Z dimension, independent pipelines can work on each XY plane.  However, at the conclusion of the XY phase, the data set must be reorganized to be distributed along X or Y, with all Z coordinates colocated.  This all-to-all problem is called "corner turning" and corresponds to swapping the high bits of the sample address with the low bits.

With two FPGA boards, each board owns half the data, but must send half of that, or one quarter of the whole, to the other board.  With four FPGA boards, each board owns one quarter of the data, but must send one quarter of that, or one sixteenth, to each other board. As the degree of parallelism grows, the data is divided, but the proportion that must be exchanged grows.

Table \ref{table:fftscaling} illustrates the effect. (Include FFTCommunications.xls here)

The overall communications problem is a combination of effects:
Data set size D - such as 128*128*128*64 bits
Parallelism N - 1/N of the data set is owned by each board
All to all - N-1/N of the data set must be communicated
Links - Each board has L links of bandwidth B
Hop count - H determined by network size and topology

So an approximate calculation of all to all performance can be made as the ratio of the amount of data to be communicated D*((N-1)/N)*Hops divided by the available communications resources N*L*B.  In short, the available resources grow linearly, but the network load grows only with hopcount, which is sublinear.

Table XXX. Network topologies
Direct connected Hopcount 1
Full bisection switched star network. Hopcount 1
Two-D torus - sqrt(N)
Three-D torus - 3/2 cube root(N)
Hypercube - 1/2 lg(N)

Perhaps the best candidate network would be a full-bisection switched network.  This configuration would require something like 4 independent 64-port 100Gbps switches connected to each of 64 FPGAs.  In this scheme, for a 128x128x128 FFT, each of 64 nodes would send one 1 4096 byte message to each other board with the load shared by 4 100 Gbps links.  The whole process should take less than 6 microseconds. 64 8-way vectorized FFT pipelines meanwhile could execute the LR force pipeline in about 41 microseconds.

Off-board communications are made available to OpenCL code as Intel's extension to OpenCL - fifo based channels.

It is certainly possible to build a general purpose network switch in OpenCL, but it is not necessary for this application.  Instead, for up to 4 FPGA boards, point to point links can be used.  For more than 4 boards, each board contains a centrally controlled switch that reads a series of control words from memory and configures the router packet by packet "route 32 words from input 1 to output 2".  The communications pattern of 3DFFT is completely regular, so the sequence of switch configurations can be precompiled.  This also avoids the need for packet headers.  Router crosspoints are simply built from OpenCL channels with specified storage.  The OpenCL compiler automatically uses FPGA block rams for implementation.

\subsection{Application Considerations}

In molecular modelling, short range forces are computed pairwise among particles, using a force model.  This leads to a nearest neighbor decomposition with halo communication to adjacent nodes in two or three dimensions, corresponding to a 2D or 3D network topology.

In the alternative, application data may be decomposed in only one dimension, into, for example XY slabs, with each node holding a range of Z coordinates.  Such a decomposition may tend to underutilize network connections in the other dimensions, but whether this is actually a problem depends on the data volume communicated to nearest neighbors and the relative tradeoff of computation to communications.

For the 3D FFT, the slab organization is very tempting, because two of the three dimensions can be computed locally without any communications.  In this case, X and Y transforms may be completed locally, and then data transposed for the Z transform.

The slab organization has an additional benefit because the X and Y transforms can be pipelined without storing the intermediate data into global memory.



 \subsection{All to All}\label{alltoall}
 
 In the previous section, we noted that the role of the All to All portion of the 3D FFT is to reorganize the dataset so that all the values for a pencil in the Z direction are colocated, so that a Z direction 1D FFT may be performed.  During X and Y phases, the dataset is split into slabs along the Z dimension.  During the Z phase, the dataset is split into slabs along the Y dimension.
 
 There are many ways to make this transition, but a very convenient solution is to interchange the low and high bits of the shape.  In the previous example, the all to all hardware changes
 
\begin{scriptsize}
 \begin{verbatim}
 A2AIn   Y4 Y3 Y2 Y1 Y0 X0 X1 X2 X3 X4 Z0 Z1 Z2 Z3 Z4
A2AOut  Z4 Z3 Z2 Y1 Y0 X0 X1 X2 X3 X4 Z0 Z1 Y2 Y3 Y4
 \end{verbatim}
 \end{scriptsize}

The wiring for 8 pipelines on one FPGA is shown in Figure \ref{fig:a2a_1_8}. In this figure the eight blocks on the left represent the 8-wide vector outputs of eight FFT pipelines, and the eight blocks on the right route data back to the respective pipelines. This can also viewed as a matrix transpose, in which the various FFT pipelines send data column wise to the All to All, and then rows are sent back to the processing pipelines. This is shown in figure \ref{fig:a2a_8_1_transpose}.  Each line on this diagram represents a 64 bit parallel bus carrying a single precision complex number at, typically 300 MHz. 


%\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\newcommand\T{\rule{0pt}{2.6ex}}       % Top strut
\newcommand\B{\rule[-1.2ex]{0pt}{0pt}} % Bottom strut
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
XYZ&Data Points&Data Bits&1&2&4&8&16&32&64 \\
$32^3$&32768&2097152&4096&2048&1024&512&256&128&64 \\
$64^3$&262144&16777216&32768&16384&8192&4096&2048&1024&512 \\
64x64x128&524288&33554432&65536&32768&16384&8192&4096&2048&1024 \\
$96^3$&884736&56623104&110592&55296&27648&13824&6912&3456&1728 \\
$128^3$&2097152&134217728&262144&131072&65536&32768&16384&8192&4096 \\
\hline
\end{tabular}%
}
\vspace{0.05pt}
\caption{Time in cycles for FFT sizes vs number of units}
\label{table:fftcycles}
\end{table}

==> networking.tex <==
\section{Networking}

Bandwidth concerns
Network topology
Overhead
Idea of centrally scheduled networking

==> outline.tex <==
\section{Outline}

section Introduction

Large scale use of MD.

Clusters of GPU based systems for throughput computing.

MD alternatives: 
CPU based
GPU based
ASIC based (Anton)
FPGA

Need for faster turnaround time -> strong scaling

MD composed of combinations of bonded forces and non-bonded.

Non-bonded forces are short range and amenable to particle in cell techniques
Direct computation of long range forces (electrostatic) do not scale well due to $N^2$

Fourier transform methods (PME) greatly reduce computation, but strong scaling is difficult due to communications requirements - no matter how you do Fourier transforms, every output depends on every input.

What's new

Availability of FPGAs with communications
Availability of FPGAs with HBM
Availability of OpenCL

Contribution of this paper:

High performance distributed 3DFFT for FPGA cluster, integrated with other MD components.
a) scalable streaming computation of FFT input
b) general method for bit dimension permutations
c) Use of HBM buffering for transposes too large for BRAM
d) overlap of communications with computation
d) numbers of processing pipelines for strong scaling
e) streaming force interpolation

section MD Background

Short version of overall problem

Longer explanation of PME

section FPGA background

HBM
Communications links
Networking
OpenCL

section FFT System Architecture


section FFT Background
3D FFT
3D FFT Scaling.  Communications and bandwidth requirements.  Sizes

Networking

Role of permutations

FFT Implementation
Design style
Attention to initiation interval and unit latency

BRAM vs HBM implementations

section FFT Integration with overall MD

Atom data
Structure parameters
Fixing FFT size
Force update records
Slabs vs cubes

section Summary and Future Work


OpenCL improvements
OpenCL access to switched communcations
MPI host program


Figure list:
=======

Complete system  (like Carlo diagram of processing pipelines)

LR processing flow  (charge spread, FFT, multiplication by greens function, IFFT, force interpolation

3D FFT
FFT Core?

Transpose unit

Typical .fft file

Performance data on single fpga FFT

Performance data on multiboard FFT

Scaling properties of FFT with distribution and communications

GPU FFT scaling

List of References
============

Plessl system  (optical switch)
Tsukuba system (Ethernet switch)

OpenCL Pipes, channels, streaming messaging interface

Lasst year's SC Paper
Feedforward FFT paper
Other FFT refs (FFTW, etc)

GPU FFT
Intel FFT

PME papers
B-Spline papers

Bit dimension permutation papers

Nallatech/Molex
Xilinx?



Work items and assignments
==================

Introduction - value of strong scaled MD to drug discovery

MD Background -
  General
  PME


Data needed
   4 board results  -Larry
   


==> pme.tex <==
\section{Particle Mesh Ewald}
In molecular modelling, the primary contributor to long-range forces are electrostatic interactions. Two particles exert forces on one another according to the product of their charges divided by the square of the distance between them. Pairwise computations become infeasible with 50,000 to 100,000 particles. Instead, the positions of particles and their charges are used to calculate a potential field using Fourier Transform methods. This is called Particle Mesh Ewald method. The overall potential is the 3D convolution of the scalar charge field with another 3D scalar field which embodies the $1/r^2$ dependency. This 3D convolution becomes a pointwise multiplication in Fourier space, which greatly reduces computational requirements. An inverse 3D FFT then produces a scalar potential field. Particle forces are then calculated by using the 3D gradient of the potential.

The processing flow of the long-range timestep is as follows:
The input data is the data set of current particle positions and charges.
The charges are spread to a 4x4x4 block of the input volume of the Fourier Transform, which will typically be in the range 32x32x32 to 128x128x128 for problems with 50,000 to 100,000 atoms. The charge spreading phase requires calculation of Cardinal B-Splines of order 4 in each dimension for each particle, according to the fractional distance of the particle between FT grid points.
The (notionally 128x128x128) FT input volume is then fed to a 3D real-to-complex FFT.
The frequency domain volume (128x128x128 complex) is pointwise multiplied by another precomputed volume representing the structure parameters. The result is then passed to a 3D complex to real inverse FFT.
The linear space result is the overall electrical potential field experienced by the particles. In a process similar to charge spreading, a 4x4x4 block of the potential space is used, via fourth order cardinal B-splines in each dimension, to calculate potential gradients in each dimension and to generte a force update record for each particle.

We have chosen to break down this processing pipeline into two major functional units. Because the charge spreading and force interpolation steps have very similar structure and do not operate at the same time, we can share a single hardware unit for these functions. The Core FFT unit is composed of two single precision complex 8 wide pipelined FFT units, with additional bit-dimension permutation units at input, output, and between the FFTs. Finally, multiple processing pipelines, each composed of a charge-spread/force-interpolation unit and a dual-FFT unit, are interconnected by an All-to-All communications structure which handles local and remote routing of data among processing pipelines. Additional small load/store units handle reads and writes from banks of high bandwidth memory. To meet bandwidth and operating frequency requirements, each processing pipeline requires 5 banks of HBM memory for about 48 GB/sec memory bandwidth per processing pipeline at 300 MHz.

The overall Molecular modelling architecture is shown in figure XXX



==> singlepage.tex <==

\section{Extended Abstract} \label{abdstract}

Molecular Dynamics (MD) simulations play a central role in physics-driven drug discovery. MD applications often use the Particle Mesh Ewald (PME) algorithm to accelerate electrostatic force computations, but efficient parallelization has proven difficult due to the high communication requirements of distributed 3D FFTs. In this paper, we present the design and implementation of a scalable PME algorithm that runs on a cluster of Intel Stratix 10 FPGAs and can handle FFT sizes appropriate to address real-world drug discovery projects (grids up to {\boldmath $128^3$}). To our knowledge, this is the first work to fully integrate all aspects of the PME algorithm (charge spreading, 3D FFT/IFFT, and force interpolation) within a distributed FPGA framework. The design is fully implemented with OpenCL for flexibility and ease of development and uses 100 Gbps links for direct FPGA-to-FPGA communications without the need for host interaction. We present experimental data up to 4 FPGAs (e.g., 206 microseconds per timestep for a 65536 atom simulation and {\boldmath $64^3$} 3D FFT), outperforming GPUs for smaller FFT sizes. Additionally, we discuss design scalability on clusters with differing topologies up to 64 FPGAs (with expected performance far greater than all known GPU implementations) and integration with other hardware components to form a complete molecular dynamics application. We predict best-case performance of 6.6 microseconds per timestep on 64 FPGAs.
